Magnetic field and prominences of the young, solar-like, ultra-rapid rotator V530 Per

We investigate signatures of magnetic fields and activity at the surface and in the prominence system of the ultra-rapid rotator V530 Per, a G-type solar-like member of the young open cluster $\alpha$~Persei. This object has a rotation period shorter than all stars with available magnetic maps. With a time-series of spectropolarimetric observations gathered with ESPaDOnS over 2 nights on the CFHT, we reconstruct the surface brightness and large-scale magnetic field of V530 Per using the Zeeman-Doppler imaging method, assuming an oblate stellar surface. We also estimate the short term evolution of the brightness distribution through latitudinal differential rotation. Using the same data set, we finally map the spatial distribution of prominences through tomography of the H\alpha emission. The brightness map is dominated by a large, dark spot near the pole, accompanied by a complex distribution of bright and dark features at lower latitudes. The magnetic field map is reconstructed as well, most of the large-scale magnetic field energy is stored in the toroidal field component. The main radial field structure is a positive region of about 500 G, at the location of the dark polar spot. The brightness map of V530 Per is sheared by solar-like differential rotation, with a roughly solar value for the difference in rotation rate between the pole and equator. \halpha~is observed in emission, and is mostly modulated by the stellar rotation period. The prominence system is organized in a ring at the approximate location of the co-rotation radius, with significant evolution between the two observing nights. V530 Per is the first example of a solar-type star to have its surface magnetic field and prominences mapped together, which will bring important observational constraints to better understand the role of slingshot prominences in the angular momentum evolution of the most active stars.

==> Tables/AllTab.tex <==
%----------> tab:obslog <-----------% 
\input{Tables/obslog}
\input{Tables/Parameters}
\input{Tables/magE.tex}
